Conflict Essences for Transformation Rules with Nested Application Conditions -- Long Version

Conflict and dependency analysis is an important static analysis tool that provides an overview of the potential interactions of (graph) transformation rules. This analysis is based on critical pairs and initial conflicts, which represent conflicting transformations in a minimal context. However, the crucial information about a conflicting transformation pair is contained in much smaller structures, called disabling/conflict essences in existing research. Recently, we introduced disabling essences for rules with application conditions which contain the information on how an application condition can be violated by another rule. In this paper, we extend the notion of disabling essences to support not only application conditions in Alternating Quantifier Normal Form, but also arbitrary nested conditions. We introduce (symbolic) conflict essences that are constructed from disabling essences and which capture the interaction between two rules. We show that a transformation pair is parallel dependent if and only if a symbolic conflict essence can be embedded into it and relate symbolic conflict essences to initial conflicts for transformation rules with application conditions. We present our results for adhesive HLR categories, which includes several types of graph-like structures.

==> imports.tex <==
\usepackage{listings}
\usepackage{graphicx}
\usepackage{enumitem}
\usepackage{import}
\usepackage[nolist]{acronym}
\input{settings/acronyms.tex}
%\usepackage{todonotes}
\usepackage[disable]{todonotes}
%\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage[style=british]{csquotes}
%\usepackage{hyperref}
%%%%%% To display ORCID Logo with link, Please add below definition and copy the ORCID_Color.eps in the manuscript package %%%%%
\makeatletter
\RequirePackage[bookmarks,unicode,colorlinks=true]{hyperref}%
   \def\@citecolor{blue}%
   \def\@urlcolor{blue}%
   \def\@linkcolor{blue}%
\def\UrlFont{\rmfamily}
\def\orcidID#1{\smash{\href{http://orcid.org/#1}{\protect\raisebox{-1.25pt}{\protect\includegraphics{figures/orcid_color-eps-converted-to.pdf}}}}}
\makeatother

% If you use the hyperref package, please uncomment the following two lines
% to display URLs in blue roman font according to Springer's eBook style:
\usepackage{xcolor}
\renewcommand\UrlFont{\color{blue}\rmfamily}
\usepackage[noabbrev,capitalise]{cleveref}
\crefname{exa}{Example}{Examples}
\crefname{lem}{Lemma}{Lemmata}
\crefname{cor}{Corollary}{Corollaries}
\crefname{defi}{Definition}{Definitions}
\crefname{thm}{Theorem}{Theorems}
\usepackage[noend]{algpseudocode}
\usepackage[Algorithm]{algorithm} 
\usepackage[most]{tcolorbox} % colored box for research challenges
\usepackage{float}
\usepackage{adjustbox}
\usepackage{cite}
\usepackage{tikz}
\usetikzlibrary{arrows,matrix}
%positioning,arrows,,calc,shapes.geometric,babel
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage{subcaption}
\usepackage{graphics}
\usepackage{graphicx, rotating}
\usepackage{siunitx}


==> settings/acronyms.tex <==
%!TEX root = ../main.tex

\begin{acronym}
	\acro{CRA}{Class Responsibility Assignment}
	\acro{DSL}{Domain-Specific Language}
	\acro{GIPS}{\textbf{G}raph-Based (M)\textbf{I}LP \textbf{P}roblem \textbf{S}pecification}
	\acro{GIPSL}{\textbf{G}raph-Based (M)\textbf{I}LP \textbf{P}roblem \textbf{S}pecification \textbf{L}anguage}
	\acro{GT}[GT]{Graph Transformation}
	\acro{ILP}[ILP]{Integer Linear Programming}
	\acro{LHS}{Left-Hand Side}
	\acro{RHS}{Right-Hand Side}
	\acro{OCL}{Object Constraint Language}
	\acro{ANF}{Alternating Quantifier Normal Form}
	\acro{NAC}{Negative Application Condition}
\end{acronym}
